Assessing Reference-Free Peer Evaluation for Machine Translation

Reference-free evaluation has the potential to make machine translation evaluation substantially more scalable, allowing us to pivot easily to new languages or domains. It has been recently shown that the probabilities given by a large, multilingual model can achieve state of the art results when used as a reference-free metric. We experiment with various modifications to this model and demonstrate that by scaling it up we can match the performance of BLEU. We analyze various potential weaknesses of the approach and find that it is surprisingly robust and likely to offer reasonable performance across a broad spectrum of domains and different system qualities.

==> extra_tables.tex <==



\begin{table*}[!htp]\centering
\scalebox{0.80}{
\begin{tabular}{lrrrrrrrrrr}\toprule
 & en-de & de-en & en-zh & zh-en & ru-en & en-ru & kk-en & en-kk & lt-en & en-lt\\
\midrule
BLEU (highest) & 46.38 & 46.86 & 19.69 & 44.03 & 46.56 & 37.18 & 33.93 & 18.68 & 37.83 & 21.60 \\
BLEU (prism) &  38.76 & 37.94 & 7.07 & 21.49 & 36.06 & 29.86 & 30.96 & 11.18 & 28.70 & 17.48 \\
\midrule
Rank & 19/25 & 12/19 & 9/15 & 14/18 & 10/17 & 7/15 & 3/14 & 5/14 & 7/14 & 7/15 \\
\bottomrule
\end{tabular}
}
\caption{} \label{tab:quality}
\end{table*}

\begin{table}[!htp]\centering
\scalebox{0.95}{
\begin{tabular}{lrr}\toprule
\textbf{LP} & \textbf{Prism-39} & \textbf{WMT-15} \\
\midrule
en-zh &	6.174 &	7.808 \\
en-fr &	6.547 &	7.607 \\
en-ru &	6.353 & 7.585 \\
en-cs &	5.795 &	7.415 \\
en-es &	6.644 &	7.181 \\
de-fr &	5.816 &	6.992 \\
en-fi &	5.450 &	6.819 \\
de-en &	6.135 &	6.654 \\
en-et &	5.348 &	6.338 \\
en-lv &	4.974 &	5.805 \\
en-lt &	5.229 &	5.803 \\
en-kk &	5.310 &	5.347 \\
en-gu &	0.000 & 4.067 \\
de-cs &	5.575 &	0.000 \\
\bottomrule
\end{tabular}}
\caption{Corpus size for overlapping language pairs from Prism-39 and WMT-15 dataset. (In logarithm space): WMT-15 has larger amount of parallel data available per language pair as compared to Prism-39, except de-cs where no parallel corpora is available in the WMT-15 dataset.} \label{tab:data1}
\end{table}

\begin{table}[!htp]\centering
\scalebox{0.95}{
\begin{tabular}{lrr}\toprule
\textbf{LP} & \textbf{WMT-15-Mono} & \textbf{Wiki-39} \\
\midrule
de &	8.440 &	7.778 \\
en &	8.301 &	8.117 \\
fr &	8.207 &	7.686 \\
lt &	8.026 &	6.595 \\
ru &	7.904 &	7.665 \\
cs &	7.858 &	6.975 \\
fi &	7.275 &	6.897 \\
kk &	7.141 &	6.524 \\
gu &	6.667 &	0.000 \\
zh &	6.334 &	7.338 \\
\bottomrule
\end{tabular}}
\caption{Corpus size for overlapping language pairs from WMT-15-Mono and Wiki-39 dataset (In Logarithm Space). } \label{tab:data2}
\end{table}


\begin{table}[!htp]\centering
\scalebox{0.80}{
\begin{tabular}{lcccccc}\toprule
\textbf{Metric} & \multicolumn{3}{c}{\textbf{Significant}}& \multicolumn{3}{c}{\textbf{Not Significant}} \\ 
& C & IC & NS & C & IC & NS \\
\midrule
\textit{All Systems} \\
BLEU & 768  & 37 & 80 & 126 & 71 & 70\\
Prism & 778 & 61 & 46 & 136 & 93 & 38\\
\textit{en-xx Systems} \\
BLEU & 411 & 25 & 53 & 38 & 25 & 26\\
Prism & 421 & 36 & 32 & 39 & 29 & 21\\
\textit{xx-en Systems} \\
    BLEU  & 285 & 8 & 20 & 67 & 40 & 33\\
Prism & 277 & 23 & 13 & 74 & 53 & 13 \\
\textit{xx-yy Systems} \\
BLEU & 72 & 4 & 7 & 21 & 6 & 11\\
Prism & 80 & 2 & 1 & 23 & 11 & 4\\
\bottomrule
\end{tabular}}
\caption{WMT19 pairwise system level comparisions: } \label{tab:pairwise}
\end{table}

% Category C-S, IC, C-NS
\begin{table}[!htp]\centering
\scalebox{0.70}{
\begin{tabular}{lcccccc}\toprule
\textbf{Metric} & \multicolumn{3}{c}{\textbf{Human-S}}& \multicolumn{3}{c}{\textbf{Human-NS}} \\ 
& C-S (\uparrow) & C-NS & IC (\downarrow)  & C-S (\uparrow) & C-NS & IC (\downarrow) \\
\midrule
\textit{All Systems} \\
BLEU &  768 & 46 & {\bf 71} & 126 & 37 & {\bf 104}\\
Prism & {\bf 778} & 28 & 79 & {\bf 136} & 22 & 109\\
\textit{en-xx Systems} \\
BLEU & 411 & 30 & 48 & 38 & 16 & {\bf 35} \\
Prism & {\bf 421} & 21 & {\bf 47} & {\bf 39} & 11 & 39\\
\textit{xx-en Systems} \\
    BLEU  & {\bf 285} & 10 & {\bf 18} & 67 & 16 & {\bf 57}\\
Prism & 277 & 7 & 29 & {\bf 74} & 8 & 58 \\
\textit{xx-yy Systems} \\
BLEU & 72 & 6 & 5 & 21 & 5 & 12\\
Prism & {\bf 80} & 0 & {\bf 3} & {\bf 23} & 3 & 12\\
\bottomrule
\end{tabular}}
\caption{WMT19 pairwise system level comparisons: Human-NS and Human-S means insignificant and significant differences according to human scores. C and IC stands for Corrent and Incorrect ranking according to metric and human scores. The {\em  Correct} category is further divided into two based on whether the metric differences were significant (C-S) or not (C-NS). } \label{tab:pairwise}
\end{table}

\begin{table*}[!htp]\centering
\scalebox{0.80}{
\begin{tabular}{lr|rrrrrrrr}\toprule
\textbf{Data} & Avg & en-cs & en-de & en-fi & en-gu & en-kk & en-lt & en-ru & en-zh  \\\midrule
Prism-39 & 0.858 &  {\bf 0.871} &	0.730 & 0.878 &  0.400 & 	0.813 &	0.939 &	{\bf 0.901} &	0.789 \\
WMT-15 & 0.840 & 0.825 &	0.530 &	0.815 &	0.423 &	0.909 &	0.914 &	0.845 &	0.774 	 \\
Prism-13 & 0.863 & 0.869 &	{\bf \underline{0.779}} & { \bf 0.891} & 0.379	& 0.820& 0.925 &	{\bf 0.901} &	0.795\\
Prism-39 + WMT-15 & \underline{0.867} & 0.862 &	0.653 &	0.854 &  0.446 &	0.860 & 	0.932 &	0.880 & 	0.789 \\
% Prism-39 + Finetune on WMT-15 & 0.861 & 0.870&	0.592&	0.838 &	0.486 &	0.899 &	0.937 &	0.878 &	0.786 \\
% Prism-13 + WMT-15 & 0.861 & 0.853 &	0.638&	0.841&	0.434&	0.837 &	0.931 &	0.868&	0.802 \\
\midrule
\textit{Adding monolingual data} \\
Prism-39 + Wiki-39 & 0.832 & 0.839 &	0.649 &	0.854 &	0.446 &	0.823	&0.917 &	0.877 &	0.757 \\
WMT-15 + WMT-15-Mono & {\bf 0.869} & 0.855	 &0.646 &	0.826 &	{\bf \underline{0.848}} &	{\bf 0.913} &	0.940 &	0.867 &	{\bf 0.793}\\
Prism-39 + WMT-15-Mono & 0.851 & 0.869 &	\underline{0.766} &	0.871 &	0.487 &	0.850 &	{\bf 0.945} &	0.892 &	0.754 \\
\midrule
Bilingual Models &  &  &0.726 & & & & 0.695 & 0.867 & 0.769\\
\bottomrule
\end{tabular}}

\vspace{0.2cm}
\scalebox{0.80}{
\begin{tabular}{lrrrrrrr|rrr}\toprule
\textbf{Data} & de-en&  fi-en & gu-en & kk-en & lt-en & ru-en & zh-en & de-cs & de-fr & fr-de \\\midrule
Prism-39 &  0.796 &  0.942 & 0.893 & 0.709 &	0.978 &	0.739 &	0.828& 0.991 &  0.882 & 0.203\\
WMT-15 &  0.815 & 0.954 & 0.918 & 0.509 &	0.986 &	0.841 &	0.835& 0.970 & 0.851 & 0.116\\
Prism-13 & {\bf \underline{0.845}} & 0.943 & 0.911 & {\bf 0.745} &	0.983 &	0.749 &	{\bf 0.836} & 0.985 & 0.863 & 0.124\\
Prism-39 + WMT-15 &  \underline{0.802} & 0.950 &  0.921 & 0.734 &	\underline{0.986} &	{\bf \underline{0.851}} &	0.810& {\bf 0.993} & 0.881 & 0.170\\
% Prism-39 + Finetune on WMT-14 &  0.812 &0.953 & 0.918 &	0.706 &	0.981 &	0.855 &	0.827  & 0.984 & 0.888 & 0.214\\
% Prism-12 + WMT-14 & 0.831 & 0.955 &0.922 &	0.711 &	0.987&	0.847 &	0.840&0.983 & 0.884 & 0.171  \\
\midrule
\textit{Adding monolingual data} \\
Prism-39 + Wiki-39 &0.742 & 0.934 & 0.907 &	0.684 &	0.975 &	0.680 & 	0.836	& 0.982 & 0.822 & 0.117\\
WMT-15 + WMT-15-Mono & \underline{0.842} & {\bf \underline{0.956}} & {\bf \underline{0.976}} &	0.584 &	{\bf 0.987} &	0.838	 & 0.824 & 0.903 & {\bf 0.890} & {\bf 0.238} \\
Prism-39 + WMT-15-Mono &  0.803 & 0.944 & \underline{0.952} &	0.680 &	0.952	& 0.722 &	0.754& 0.972 & 0.875 & 0.233 \\
\midrule
Bilingual Models & 0.801 & & & & 0.862 & 0.650 & 0.826 & & & \\
\bottomrule
\end{tabular}
}
\caption{Effect of training data. Significant improvement over baseline ``Prism-39'' systems are underlined. \footnote{Even though the average correlation is higher for WMT-15 + WMT-15-Mono than Prism-39 + WMT-15, it is not statistically significant as compared to the baseline Prism-39 results. We attribute this to increase in correlation for en-gu but degradation in other language pairs such as en-de, en-fi, kk-en etc.}} \label{tab:corpora}
\end{table*}



%%%% Subset Tables

% We first compare ``Prism-src'' with our reproduced target-side tagged model ``Prism-39-trg2xx''. We attribute the difference in average correlation (Avg, $-0.008$) to the  difference in optimization strategy and the effective batch size used during training.  We obtain comparable average correlation with ``Prism-src'' using language-id tagging on the source side (``Prism-39-src2xx''), where our model obtains significantly better correlation for low resource language pairs such as en-lt ($+0.031$) and en-fi ($+0.020$), but has lower correlation for medium resource language such as en-de ($-0.024$) and fr-de ($-0.063$). 

\begin{table}[!htp] \centering
\scalebox{0.80}{
\begin{tabular}{lrrrr}\toprule
\textbf{Metric} & All & en-xx & xx-en & xx-yy \\\midrule
BLEU & 0.911 & 0.917 & 0.921 & 0.838	 \\
CHRF & 0.933  & 0.937 & 0.919 & 0.954 \\
\midrule
UNI+ & 0.808 \\
Yisi-2 & 0.487 & \\
Prism & {\bf 0.861} & 0.814 & 0.887 & 0.911\\
\midrule
Prism-trg2xx & 0.853 & 0.812 & 0.872 & 0.907\\
Prism-src2xx & 0.858 &  0.822 & 0.871 & 0.914\\
\bottomrule
\end{tabular}}
\caption{Baseline results. All numbers are average system-level correlations.}
\end{table}

% We study the effect of using WMT corpora for training the multilingual MT system and contrast it against the Prism corpora used for training our baseline model (See Table~\ref{tab:data1} for details).

% Table~\ref{tab:corpora} shows that the scores derived from the multilingual model trained on WMT corpora (WMT-15) achieves lower correlation ($-0.034$) than the model that is trained on Prism corpora (``Prism-39''). Since, the model is also trained on many more languages, we compare the average correlation of the multilingual model trained only on the subset of languages available in the WMT dataset, referred to as ``Prism-13''.\footnote{No parallel data is available in Prism corpora for hi and gu.} This model improves average correlation over both the models trained on WMT corpora ($+0.004$) and Prism dataset ($+0.038$). Specifically, we observe improved correlation for en-de ($+0.049$) and de-en ($+0.049$) as compared to the Prism-39 model. Furthermore when using all the corpora (Prism and WMT) available, we improve the correlation score for to-English language pairs, de-en, gu-en and ru-en which can be attributed to the en-centric nature of the WMT dataset.

% \subsubsection*{Adding Monolingual Data via MASS}
% Inspired by the improvements in translation quality for low-resource languages via the addition of monolingual corpora \cite{siddhant-etal-2020-leveraging}, we study the effect of adding monolingual corpora to the training dataset using the MASS denoising objective. We study three different scenarios to disambiguate the effect of domain and the addition of monolingual dataset :
% \begin{enumerate}
%     \item Adding general domain monolingual dataset to the Prism parallel corpora (Prism-39 + Wiki-39)
%     \item Adding in-domain monolingual dataset to WMT training corpora (WMT-15 + WMT-15-Mono)
%     \item Adding in-domain monolingual dataset to the Prism parallel corpora (Prism-39 + WMT-15-Mono)
% \end{enumerate}

% From Table~\ref{tab:corpora}, we can observe that adding general domain monolingual dataset to Prism-39 corpora (2) hurts correlation scores across the board. We do observe slight improvement in correlation for en-xx language pairs: en-de, en-gu and en-kk   when adding in-domain WMT training dataset to Prism-39 corpora (1). We see maximum gains in average correlation ($+0.029$) when in-domain monolingual dataset is added to the WMT corpora due to increase in correlation for en-gu/gu-en.

\begin{table}[!htp] \centering
\scalebox{0.75}{
\begin{tabular}{lrrrr}\toprule
\textbf{Data} & All & en-xx & xx-en & xx-yy \\\midrule
Prism-39 & 0.858 &  0.822 & 0.871 & 0.914 \\
WMT-15 & 0.840 & 0.776 & 0.890 & 0.854 \\
Prism-13 & 0.863 & 0.828 & 0.888 & 0.888\\
Prism-39 + WMT-15 & \underline{0.867} & 0.811 & 0.896 & 0.923 \\
\midrule
\textit{Adding monolingual data} \\
Prism-39 + Wiki-39  & {\bf 0.870} & 0.839 & 0.910 & 0.818 \\
Prism-39 + WMT-15-Mono & 0.851 & 0.831 & 0.863 & 0.874 \\
% \midrule
% Bilingual Models & \\
\bottomrule
\end{tabular}}
\caption{Effect of training data. Significant improvement over baseline ``Prism-39'' systems are underlined. \footnote{Even though the average correlation is higher for WMT-15 + WMT-15-Mono than Prism-39 + WMT-15, it is not statistically significant as compared to the baseline Prism-39 results. We attribute this to increase in correlation for en-gu but degradation in other language pairs such as en-de, en-fi, kk-en, de-cs etc.}} \label{tab:corpora}
\end{table}

\begin{table}[!htp] \centering
\scalebox{0.75}{
\begin{tabular}{lrrrr}\toprule
\textbf{Metric} & All & en-xx & xx-en & xx-yy \\\midrule
BLEU & {\bf 0.911}  & 0.917 & 0.921 & 0.838 \\
Big & 0.808 & 0.745 & 0.838 & 0.885\\
Prism & 0.858  &  0.822 & 0.871 & 0.914 \\
Massive & 0.883 & 0.858 & 0.890 & 0.927 \\
\bottomrule
\end{tabular}}
\caption{Effect of Model capacity.
%Results that are not significantly outperformed by any other method are underlined.
} \label{tab:capacity}
\end{table}


\begin{table*}[!htp]\centering
\scalebox{0.80}{
\begin{tabular}{lrrrr}\toprule
\textbf{Aggregation Method} & All & en-xx & xx-en & xx-yy\\\midrule
Mean & 0.883 & 0.858 & 0.890 & 0.927  \\
Std-dev &  0.882 & 0.847 & 0.903 & 0.919 \\
Median & 0.870 & 0.859 & 0.876 & 0.887\\
Min  & 0.872 & 0.840 & 0.895 & 0.896\\
\midrule
MC-dropout (Mean) & 0.877 & 0.847 & 0.888 & 0.926	\\
MC-dropout (Std-dev)  & 0.855 & 0.864 & 0.820 & 0.904 \\
SP-Norm (Mean) &  0.884 & 0.861 & 0.892 & 0.924\\
\midrule
Confidence threshold & {\bf 0.886} \\
\bottomrule
\end{tabular}}

\caption{Scoring methods. Significant improvements over baseline {\em Mean} systems are underlined.} \label{tab:alternate}
\end{table*}

% We study the impact of varying the model capacity on the correlation scores with human judgements.  Decreasing the capacity of the model hurts average correlation score by a significant margin ($-0.051$), as the model is not provided with sufficient capacity to learn from the training dataset, whereas, increasing the model capacity improves the correlation significantly, across all language pairs, achieving parity with BLEU.

% Aggregating token-level probabilities via standard deviation results in comparable average correlation as mean (Table~\ref{tab:alternate}). However, we do not observe any consistent pattern across language pairs when using different schemes for combining token-level probabilities.

% Unlike prior results on using model-uncertainty based features, we do not observe any gains in the average correlation from using the unbiased Monte-Carlo estimate. This could be attributed to the observation that dropout is applied to an external model and not to the model that generated the output. On the other hand, our proposed data-uncertainty based metric, SP-Norm, improves the  correlation significantly for en-kk and en-zh.


% Category C-S, IC, C-NS
% \begin{table}[!htp]\centering
% \scalebox{0.70}{
% \begin{tabular}{lcccccc}\toprule
% \textbf{Metric} & \multicolumn{3}{c}{\textbf{Human-S}}& \multicolumn{3}{c}{\textbf{Human-NS}} \\ 
% & C-S (\uparrow) & C-NS & IC (\downarrow)  & C-S (\uparrow) & C-NS & IC (\downarrow) \\
% \midrule
% \textit{All Systems} \\
% BLEU &  768 & 46 & {\bf 71} & 126 & 37 & {\bf 104}\\
% Prism & {\bf 778} & 28 & 79 & {\bf 136} & 22 & 109\\
% \textit{en-xx Systems} \\
% BLEU & 411 & 30 & 48 & 38 & 16 & {\bf 35} \\
% Prism & {\bf 421} & 21 & {\bf 47} & {\bf 39} & 11 & 39\\
% \textit{xx-en Systems} \\
%     BLEU  & {\bf 285} & 10 & {\bf 18} & 67 & 16 & {\bf 57}\\
% Prism & 277 & 7 & 29 & {\bf 74} & 8 & 58 \\
% \textit{xx-yy Systems} \\
% BLEU & 72 & 6 & 5 & 21 & 5 & 12\\
% Prism & {\bf 80} & 0 & {\bf 3} & {\bf 23} & 3 & 12\\
% \bottomrule
% \end{tabular}}
% \caption{WMT19 pairwise system level comparisons: Human-NS and Human-S means insignificant and significant differences according to human scores. C and IC stands for Corrent and Incorrect ranking according to metric and human scores. The {\em  Correct} category is further divided into two based on whether the metric differences were significant (C-S) or not (C-NS). } \label{tab:pairwise}
% \end{table}


\begin{table*}[!htp]\centering
\scalebox{0.80}{
\begin{tabular}{lrrrr|rrrr}\toprule
\textbf{Data} &en-de & en-lt & en-ru & en-zh  & de-en& lt-en & ru-en & zh-en \\\midrule
BLEU & 0.806 & 0.986 & 0.946 & 0.802 & 0.794 & 0.985 & 0.812 & 0.808 \\
Prism-39 &  0.730 & 0.939 & 0.901 & 0.789 & 0.796 &	0.978 &	0.739 &	0.828\\
\midrule
Bilingual Models  &0.726 & 0.695 & 0.867 & 0.769& 0.801 & 0.862 & 0.650 & 0.826 \\
\midrule
Competition-grade &  0.913 & \\
\bottomrule
\end{tabular}
}
\caption{Effect of training data. Significant improvement over baseline ``Prism-39'' systems are underlined.} \label{tab:bivsmulti}
\end{table*}
